Staged trees and asymmetry-labeled DAGs

Bayesian networks are a widely-used class of probabilistic graphical models capable of representing symmetric conditional independence between variables of interest using the topology of the underlying graph. For categorical variables, they can be seen as a special case of the much more general class of models called staged trees, which can represent any type of non-symmetric conditional independence. Here we formalize the relationship between these two models and introduce a minimal Bayesian network representation of the staged tree, which can be used to read conditional independences in an intutitive way. A new labeled graph termed asymmetry-labeled directed acyclic graph is defined, whose edges are labeled to denote the type of dependence existing between any two random variables. We also present a novel algorithm to learn staged trees which only enforces a specific subset of non-symmetric independences. Various datasets are used to illustrate the methodology, highlighting the need to construct models which more flexibly encode and represent non-symmetric structures.

==> tables/results_edges.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Wed Sep 28 09:06:08 2022
\begin{table}[ht]
\centering
\scalebox{0.5}{
\begin{tabular}{lrrrrrrrrrr}
  \toprule
 & DAG edges & total & context & partial & context/partial & local & total CST & partial CST & context/partial CST & local CST \\ 
  \midrule
abalone & 20 & 5 & 10 & 0 & 1 & 4 & 9 & 0 & 1 & 0 \\ 
  Asym & 4 & 1 & 1 & 0 & 0 & 2 & 3 & 0 & 0 & 0 \\ 
  bodyfat & 23 & 6 & 7 & 0 & 0 & 10 & 14 & 0 & 0 & 0 \\ 
  breast\_cancer\_wisconsin & 15 & 7 & 6 & 0 & 0 & 2 & 8 & 0 & 0 & 0 \\ 
  breast\_cancer & 6 & 3 & 0 & 3 & 0 & 0 & 6 & 0 & 0 & 0 \\ 
  cachexia & 6 & 4 & 0 & 2 & 0 & 0 & 6 & 0 & 0 & 0 \\ 
  car & 5 & 0 & 0 & 5 & 0 & 0 & 5 & 0 & 0 & 0 \\ 
  chestSim500 & 6 & 4 & 2 & 0 & 0 & 0 & 4 & 0 & 0 & 0 \\ 
  credit\_card & 33 & 5 & 13 & 4 & 1 & 10 & 12 & 1 & 1 & 0 \\ 
  eeg & 59 & 4 & 40 & 0 & 0 & 15 & 13 & 0 & 0 & 0 \\ 
  energy1 & 9 & 8 & 1 & 0 & 0 & 0 & 8 & 0 & 0 & 0 \\ 
  energy2 & 9 & 7 & 2 & 0 & 0 & 0 & 7 & 0 & 0 & 0 \\ 
  FallEld & 4 & 0 & 1 & 2 & 0 & 1 & 3 & 0 & 0 & 0 \\ 
  fertility & 2 & 1 & 0 & 1 & 0 & 0 & 2 & 0 & 0 & 0 \\ 
  house\_votes & 26 & 9 & 11 & 0 & 0 & 6 & 11 & 0 & 0 & 0 \\ 
  indian\_liver & 14 & 7 & 0 & 5 & 0 & 2 & 11 & 0 & 0 & 0 \\ 
  iris & 4 & 3 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 \\ 
  magic04 & 26 & 6 & 5 & 8 & 5 & 2 & 16 & -3 & 5 & 0 \\ 
  monks1 & 1 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 
  monks2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
  monks3 & 3 & 2 & 0 & 1 & 0 & 0 & 2 & 0 & 0 & 0 \\ 
  nursery & 9 & 0 & 0 & 6 & 3 & 0 & 7 & -1 & 3 & 0 \\ 
  PhDArticles & 4 & 3 & 0 & 1 & 0 & 0 & 4 & 0 & 0 & 0 \\ 
  Pokemon & 1 & 1 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 \\ 
  post\_operative & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
  puffin & 3 & 3 & 0 & 0 & 0 & 0 & 3 & 0 & 0 & 0 \\ 
  reinis & 6 & 2 & 2 & 0 & 0 & 2 & 4 & 0 & 0 & 0 \\ 
  tae & 3 & 1 & 0 & 2 & 0 & 0 & 3 & 0 & 0 & 0 \\ 
  tic\_tac\_toe & 13 & 2 & 0 & 11 & 0 & 0 & 9 & 0 & 0 & 0 \\ 
  Titanic & 5 & 3 & 1 & 1 & 0 & 0 & 4 & 0 & 0 & 0 \\ 
  voting & 26 & 9 & 11 & 0 & 0 & 6 & 11 & 0 & 0 & 0 \\ 
   \bottomrule
\end{tabular}
}
\end{table}


==> tables/results_nice_small.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Thu Sep 29 16:20:59 2022
\scalebox{0.8}{
\begin{tabular}{rrlrrrrr}
  \toprule
 & variables & Edg. ALDAG-ST & BIC DAG & BIC ST & time DAG & time ST & time ALDAG \\ 
  \midrule
abalone & 9 & (5,10,0,0,6) & 29090.40 & 28895.06 & 0.04 & 0.08 & 0.01 \\ 
  breastcancer & 10 & (4,0,3,0,0) & 4644.20 & 4594.08 & 0.01 & 1.51 & 0.25 \\ 
  creditapproval & 14 & (10,3,0,0,2) & 9881.28 & 9861.87 & 0.02 & 1.79 & 0.35 \\ 
  housevotes & 17 & (9,11,0,0,6) & 3538.93 & 3480.58 & 0.02 & 3.07 & 0.67 \\ 
  indianliver & 11 & (10,1,0,0,4) & 6984.16 & 6966.59 & 0.02 & 0.06 & 0.02 \\ 
  nursery & 9 & (0,0,5,3,0) & 252566.46 & 251922.28 & 0.06 & 1.69 & 0.11 \\ 
  phdarticles & 6 & (3,2,1,0,0) & 8371.68 & 8356.90 & 0.01 & 0.01 & 0.00 \\ 
  tic-tac-toe & 10 & (1,0,12,0,0) & 19276.60 & 18995.57 & 0.02 & 0.64 & 0.08 \\ 
  titanic & 4 & (0,1,3,0,1) & 10502.28 & 10451.72 & 0.01 & 0.03 & 0.00 \\ 
   \bottomrule
\end{tabular}
}

